An LS-Decomposition Approach for Robust Data Recovery in Wireless Sensor Networks

Wireless sensor networks are widely adopted in military, civilian and commercial applications, which fuels an exponential explosion of sensory data. However, a major challenge to deploy effective sensing systems is the presence of {\em massive missing entries, measurement noise, and anomaly readings}. Existing works assume that sensory data matrices have low-rank structures. This does not hold in reality due to anomaly readings, causing serious performance degradation. In this paper, we introduce an {\em LS-Decomposition} approach for robust sensory data recovery, which decomposes a corrupted data matrix as the superposition of a low-rank matrix and a sparse anomaly matrix. First, we prove that LS-Decomposition solves a convex program with bounded approximation error. Second, using data sets from the IntelLab, GreenOrbs, and NBDC-CTD projects, we find that sensory data matrices contain anomaly readings. Third, we propose an accelerated proximal gradient algorithm and prove that it approximates the optimal solution with convergence rate $O(1/k^2)$ ($k$ is the number of iterations). Evaluations on real data sets show that our scheme achieves recovery error $\leq 5\%$ for sampling rate $\geq 50\%$ and almost exact recovery for sampling rate $\geq 60\%$, while state-of-the-art methods have error $10\% \sim 15\%$ at sampling rate $90\%$.

==> Sections/LSDecomposition.tex <==
   \begin{table*} \label{LS_table}\centering
   \caption{Variants of LS-Decomposition.}
   \begin{tabular}{|c|c|c|c|c|c|c|c|}
   \hline
   Low-rank & Sparse & Noise & Partial & Objective & Relaxation  & Constraints & Ref. \\
   \hline\hline
   $\surd$  &        &       & $\surd$ & min $rank(L)$ & min $||L||_{*}$ & $\mathcal{P}_{\mathcal{O}}(L)=\mathcal{P}_{\mathcal{O}}(R)$ & \cite{Candy2009}\cite{Tao2010}\\
   \hline
   $\surd$ &         & $\surd$  & $\surd$ & min $rank(L)$ & min $||L||_{*}$ & $ || \mathcal{P}_{\mathcal{O}}(L-R)||_F \leq \delta$ & \cite{candes2006near}\\
   \hline
   $\surd$ & $\surd$ &  &  & min $rank(L) + \lambda ||S||_0$ & min $||L||_{*} + \lambda ||S||_1$ & $ L + S = R$ & \cite{Wright2011} \\
   \hline
   $\surd$ & $\surd$ &  & $\surd$ & min $rank(L) + \lambda ||S||_0$ & min $||L||_{*} + \lambda ||S||_1$ & $\mathcal{P}_{\mathcal{O}}(L+S) = \mathcal{P}_{\mathcal{O}}(R)$ & \cite{Wright2011} \\
   \hline
   $\surd$ & $\surd$ & $\surd$ &  & min $rank(L) + \lambda ||S||_0$ & min $||L||_{*} + \lambda ||S||_1$ & $||L+S - R||_F \leq \delta$ & P1 \\
   \hline
   $\surd$ & $\surd$ & $\surd$ & $\surd$ & min $rank(L) + \lambda ||S||_0$ & min $||L||_{*} + \lambda ||S||_1$ & $ ||\mathcal{P}_{\mathcal{O}}(L+S-R) ||_F \leq \delta $ & P2 \\
   \hline
   \end{tabular}\vspace{-3 mm}
   \end{table*}

\section{The Framework of LS-Decomposition}

  In this section, we introduce the framework of LS-Decomposition. First, we give an overview of its variants. For completeness, we present our main results, comparing with a related existing result.
  
\subsection{Overview}

  The are several variants of LS-Decomposition, matrix completion is also related, which can be seen from Table X.
  

\subsection{Main Results}

  Our results:

  P1 is discuss in \cite{Wright2010Stable}. About the relaxation:
  \begin{equation}
   \begin{split}
   &\langle \hat{L}, \hat{S}\rangle = \min\limits_{L,S}~~||L||_{*} + \lambda ||S||_1, \\
   &s.t.~~||R-L-S||_F \leq \delta
   \end{split}
   \end{equation}

  The results:
  \begin{theorem}
  (\cite{Wright2010Stable}) Suppose $L $ obeys (\ref{LS_condition}), the support of $S$ is uniformly distributed, and
  \begin{equation}
  rank(L) \leq \rho_r n \mu^{-1}(logn)^{-2}, ~\text{and}~k \leq \rho_s n^2
  \end{equation}
  with $n=max(n_1,n_2)$, $\rho_r, \rho_s$ begin sufficiently small numerical constraints. Then with high probability
  \end{theorem}














==> Sections/Simulation.tex <==
\section{Simulation Results}

\subsection{Recovery }
